Cooperative Tracking of Cyclists Based on Smart Devices and Infrastructure

In future traffic scenarios, vehicles and other traffic participants will be interconnected and equipped with various types of sensors, allowing for cooperation based on data or information exchange. This article presents an approach to cooperative tracking of cyclists using smart devices and infrastructure-based sensors. A smart device is carried by the cyclists and an intersection is equipped with a wide angle stereo camera system. Two tracking models are presented and compared. The first model is based on the stereo camera system detections only, whereas the second model cooperatively combines the camera based detections with velocity and yaw rate data provided by the smart device. Our aim is to overcome limitations of tracking approaches based on single data sources. We show in numerical evaluations on scenes where cyclists are starting or turning right that the cooperation leads to an improvement in both the ability to keep track of a cyclist and the accuracy of the track particularly when it comes to occlusions in the visual system. We, therefore, contribute to the safety of vulnerable road users in future traffic.

==> sections/method_basic_movement_forecast.tex <==
\subsection{Movement Primitive Detection}
\label{subsec:movement_primitive_detection}
The movement primitive recognition is situated in the first stage of the intention detection process. The focus of this section is on the early detection of cyclist movement types. This is realized by a classification of the 
current movement primitive at discrete points in time with a 
frequency of $100\,$Hz. In this work, two methods for the detection of movement primitives are realized. The first method is realized by human activity recognition techniques \cite{Bulling2014THA} based on the gyroscope and accelerometer sensory data, which is nowadays available on nearly every smartphone. The second method is based on head trajectories of the cyclist extracted from the stereo camera system at the infrastructure. In order to comply with the sampling rate of the 
smart device, the trajectories resulting from the camera measurements are oversampled to $100\,$Hz.

The gyroscope allows to detect rotating movements, such as pedaling, 
whereas the accelerometer is better suited to detect linear movements, 
e.g. forward movements. Furthermore, the accelerometer measurements are gravity compensated. 
Both, the gyroscope and the linear acceleration sensor measurements are 
rotated into the world coordinate frame using the estimated attitude of the smart device. 
Rotational invariance is achieved by consideration of the magnitudes in geographic north and east of the rotated sensor.
Moreover, the sensor measurements in the vertical direction are considered. 
GPS values are not considered, since they are noisy (due to multipath effects in urban areas and even absence of signal) 
and their sample frequency is to low to detect fast changes in the movements ($5\,$Hz) of the cyclist.

Features for classification are extracted from the rotated sensor measurements, i.e. time series, using sliding window techniques. 
A schematic of the performed steps for movement primitive detection based on smart devices and head trajectories is 
depicted in Fig.~\ref{fig:recognition_pipeline}.
The features extracted from the sliding windows of the smart device activity data are the mean, variance, the signals' energy~\cite{Lau2010} as well as Pearson correlations between different sensor signals in the window. Three different window lengths are considered: $0.05\,$s, $0.2\,$s and $0.5\,$s.
Moreover, polynomial and Fourrier coefficients up to the $5$th degree are extracted~\cite{Fuchs2010}.
Additionally, a coarse velocity estimate based on the smart devices inertial sensors is considered.
The past velocity measurements are approximated using polynomials with orthogonal basis 
of degree $3$ and $5$ in a sliding window manner with window length of $0.5\,$s and $2.0\,$s, respectively.
In order to reduce the dimensionality and increase the generalization performance, a recursive feature selection procedure 
using a linear support vector machine~\cite{Zhu2003SVM} is performed. This reduces the number of features from $147$ to $5$. 

\begin{figure} 
	\centering
%	\includegraphics[width=0.6\textwidth, clip, trim=50 60 100 105]{"images/har_pipeline"}
	\caption{Process for movement primitive detection based on smart device and head trajectories.}
	\label{fig:recognition_pipeline}
	\vskip -4mm
\end{figure}

The infrastructure-based detection of the cyclists' movement primitive is based on the cyclist's head trajectory.
In order to achieve translational and rotational invariance, only the velocity magnitudes in the $x-y$ plane are considered.
Additionally, the vertical component of the velocity is considered. This allows to detect the vertical head movement as an early 
indicator of the cyclist's intention to start. Polynomials with orthogonal basis describing the shape of the trajectory are used as features.
Three different window length $0.3\,$s, $0.5\,$s and $1.0\,$s with polynomials up to the $3$rd degree are considered. 
The total number of $30$ features is again reduced by feature selection to $6$ essential features.

Classification is done using a supervised learning techniques. Therefore, support vector machines (SVM) 
with a radial basis function kernel are used~\cite{Bishop2006PRM}. 
The classifier outputs probabilities, i.e. a probabilistic interpretation of the classifiers certainty. 
%in order to be used for the forecasting models predictions. 
Therefore, a probability calibration using a logistic sigmoid is performed~\cite{Niculescu-Mizil2005PGP}. 

In order to optimize the classifier, such that it detects movement primitives as early as possible, training samples are weighted.
This is a decay of weights toward the starting point, samples which are $0.3\,$s before the starting point are weighted less. 
Directly after the starting point the weights are $1$ again. Additionally, a general class weight scaling is performed, 
e.g. the starting class is assigned a higher weight. The latter weighting is only used for training of the classifier.
The class weight parameter $cl_{w}$, the penalty term $C$, and the kernel coefficient $\gamma$ of the SVM are optimized by a grid search according to the weighted F1 score under consideration of the delay. 
The model selection is performed as a multi-target optimization procedure trading off both criteria.

\subsection{Cooperative Movement Primitive Detection}
\label{sec:cooperative_mp_pred}
Cooperation on the level of movement primitive detections is achieved by a stacking ensemble method
using another meta classifier~\cite{Zhou2012EMF}.
It is also situated in the first stage of 
the intention detection process.
A schematic of this cooperative process is depicted in Fig.~\ref{fig:CooperativeIntentionForecast}.
The meta classifier combines the detections of the smart device and the infrastructure. 
Therefore, it uses the probabilities $P(Start)$ of both as well as the past velocity measurements extracted from the head trajectory of the tracked VRU as input. The latter one allows the classifier to detect the current context and to select or weight between the models in order to improve the movement primitive detection.

The probabilities are approximated using polynomials in a sliding window manner~\cite{Fuchs2010} using a time window of $0.3\,$s each. This allows to account for missing or lagged values, e.g. due to communication delays or losses. Moreover, due to the usage of the orthogonal base polynomials also 
the trend of the classifier probability outputs of smart device and infrastructure  is incorporated. 
The features describing the velocity of the head are 
the same as used before in Sec.~\ref{subsec:movement_primitive_detection}.
The coefficients of the polynomials are used as inputs of a meta classifier, realized using an SVM with a radial basis kernel and a logistic unit to output proper probabilities. The model is optimized according to the F1 score and the delay.

\begin{figure}
	\centering
	\includegraphics[width=0.52\textwidth, clip, trim=110 20 80 20]{"images/CooperativeIntentionForecast"}
	\caption{Stage 1: Cooperative starting movement primitive detection.}
	\label{fig:CooperativeIntentionForecast}
	\vskip -4mm
\end{figure}
%The MLP is optimized according to minimize the log-loss, i.e. to correctly predict the current motion primitive.
%The fusion model is optimized using adam stochastic gradient descent algorithm ({\color{magenta}reference}).



==> sections/method_evaluation.tex <==
\subsection{Evaluation}
\label{sec_method_evaluation}

\subsubsection{Movement Primitive Detection}
\ \newline
Models for starting motion detection have to 
trade off between the sensitivity of detecting the starting motion as early as possible while keeping the number of false detections low.
Therefore, movement primitive detection is evaluated using a weighted version of the F1 score (as the harmonic mean between precision and recall) and the average starting detection delay. The delay is defined as the average time after the ground truth starting point at which the classifier detects the starting motion with an accuracy of at least $90\,\%$. 
Weighted F1 score refers to the decayed sample weight just before the cyclist's start. This is based on the intuition that 
detecting the starting class little to early is better than predicting it late. 
The models are trained and evaluated using $5$ fold cross validation over the test subjects.

\subsubsection{Trajectory Forecast}
\ \newline To evaluate the trained networks and the combined approach for trajectory forecast, we compared the performance of the newly trained models to an MLP trained using trajectories of all motion types, as described in~\cite{Zernetsch.2016}. 
The performance was measured using the Average Euclidean Error ($\mathit{AEE}$,~\cite{Li.Zhao2001}) and the Average Specific Average Euclidean Error ($\mathit{ASAEE}$,~\cite{Goldhammer.2016}). The calculation of the ($\mathit{AEE}$ for a certain forecast horizon $t_\mathrm{f}$ is described by Eq.~\ref{eq:AEE}, with the number of samples $N$, the forecast position $(\hat{x}_{t_\mathrm{f}},\, \hat{y}_{t_\mathrm{f}})$ and the corresponding ground truth $(x_{t_\mathrm{f},\mathrm{GT}},\, y_{t_\mathrm{f},\mathrm{GT}})$:

\begin{equation}
\begin{split}
	&AEE(t_\mathrm{f}) = \\
	&\frac{1}{N} \sum_{i=1}^{N} \sqrt{ (\hat{x}_{t_\mathrm{f}}(i) - x_{t_\mathrm{f},\mathrm{GT}}(i))^2 + (\hat{y}_{t_\mathrm{f}}(i) - y_{t_\mathrm{f},\mathrm{GT}}(i))^2 }.
	\label{eq:AEE}
\end{split}
\end{equation}

To evaluate the forecasts at different prediction times, the $\mathit{ASAEE}$, introduced by Goldhammer et al.~\cite{Goldhammer.2016}, was used:

\begin{equation}
	ASAEE = \frac{1}{K} \sum_{k=1}^{K} \frac{AEE(T_{\mathrm{p},k})}{T_{\mathrm{p},k}}
	\label{eq:ASAEE}
\end{equation}

Where $K$ is the number of discrete time steps of a time span $T_\mathrm{p}$ and $k$ as the index of the time span.

==> sections/method_overall.tex <==
\subsection{Cooperative Trajectory Forecast}
\label{sec_method_overall}
The second stage of the intention detection process is completed by the cooperative trajectory forecast. 
It is realized by a soft gating approach, weighting  
the waiting and starting forecast model in an additive fashion. A schematic of this process is depicted in Fig~\ref{fig:stage2}. 
The cooperative trajectory forecast for a particular prediction time $t_\mathrm{c}$ is formally 
defined in the following equation:

\begin{align}
y \left(t_\mathrm{c} \right) = &g \left( x_{t_\mathrm{c}}^\mathrm{w} \right) \cdot f_\mathrm{wait} \left( t_\mathrm{c}, x_{t_\mathrm{c}} \right) \\ 
&\left( 1 - g \left( x_{t_\mathrm{c}}^\mathrm{w} \right)\right) \cdot f_\mathrm{start} \left( t_\mathrm{c}, x_{t_\mathrm{c}} \right) \nonumber
\label{eq:Fusion}
\end{align}

The gating function $g$ depends on the movement primitives computed either by the smart device,
camera, or the combination of both.
It implements the model combination by weighting 
between the forecasts of the waiting and starting forecast model ($f_\mathrm{wait}$ and $f_\mathrm{start}$, 
respectively) at time $t_\mathrm{c}$. Moreover, $x_{t_\mathrm{c}}^\mathrm{w}$ denotes the input feature vector for the model fusion, whereas 
$x_{t_\mathrm{c}}$ denotes the input for the forecasting models.

The probability output generated by the movement primitive classifier (cf. Section~\ref{sec:cooperative_mp_pred}) is directly used as a gating function to weight between the predicted forecasting models. The probability is the product of the cooperative movement primitive detection. 

\begin{figure}[t]
	\includegraphics[width=0.49\textwidth,  clip, trim=0 180 370 80]{images/EnsembleForecast.pdf}
	\caption{Stage 2: Ensemble forecast approach using two models with adaptive gating function to weight the models predictions.}
	\label{fig:stage2}
	\vskip -0.3cm
\end{figure}



==> sections/method_prediction.tex <==
\subsection{Trajectory Forecast}
%\label{sec_method_cv}
The trajectory forecast of a cyclist belongs to the second stage of the intention detection process.
To forecast the future positions of the cyclist, the measured cyclist positions over the last second are transformed from 2D world coordinates into the ego coordinate system of the cyclist and are derived numerically to obtain the longitudinal and lateral velocities. The velocities are split into different temporal windows (Fig.~\ref{fig:MLP_IN_OUT}: gray segments) and are approximated with orthogonal base polynomials. The polynomial coefficients are used as input of two MLPs, one trained for waiting and one trained for starting motions. The output of the MLPs are the coefficients of polynomials, which represent the forecast longitudinal and lateral cyclist velocities over a certain forecast horizon in different temporal windows (Fig.~\ref{fig:MLP_IN_OUT}: blue segments). The velocities are reconstructed by evaluation of the coefficients, and through numerical integration of the velocities the forecast positions are retrieved. The output of both networks are combined as described in Section \ref{sec_method_overall}.

In~\cite{Zernetsch.2016} a single MLP was trained using cyclist trajectories of all motion types. For this work two networks were trained, one model for waiting ($f_\mathrm{wait}$) and one model for starting ($f_\mathrm{start}$). The reason to separate the forecast of waiting and starting motions is to reduce the forecast error, especially of starting motions. Various movements of cyclists during the waiting phase (e.g. swaying back and forth or leaning over the handlebar) lead to a decreased performance of the network described in~\cite{Zernetsch.2016} when it comes to forecasting starting motions since these movements look similar to starting, but they do not result in a large change of the cyclist velocity.

{
	\setlength{\abovecaptionskip}{5pt plus 3pt minus 3pt}
	\begin{table}[h]
%			\vskip -3mm
		\begin{center}
			\caption{Configuration of polynomials used to train the MLP.} 
			\begin{tabular}{| c | c | c | c |}
				\hline
				Polynomial & Degree & Start Time & Length \\ \hline
				$P_{in1}$ & $2$ & $-1.0\,$s & $0.5\,$s \\ \hline
				$P_{in2}$ & $3$ & $-0.5\,$s & $0.5\,$s \\ \hline
				$P_{out1}$ & $3$ & $0.0\,$s & $0.5\,$s \\ \hline
				$P_{out2}$ & $3$ & $0.5\,$s & $0.5\,$s \\ \hline
				$P_{out3}$ & $3$ & $1.0\,$s & $0.5\,$s \\ \hline
				$P_{out4}$ & $3$ & $1.5\,$s & $0.5\,$s \\ \hline
				$P_{out5}$ & $3$ & $2.0\,$s & $0.5\,$s \\ \hline
			\end{tabular}
			\label{tab:polynomials}
		\end{center}	
	
	\end{table}
}

To train the networks, 124 starting and 124 waiting scenes of uninstructed cyclists were used. The motion types were labeled manually  where the beginning of a starting motion $t_\mathrm{s}$ is defined as the first movement and the beginning of waiting $t_\mathrm{w}$ is defined as the last movement of the rear wheel of the bicycle. To train the starting network, trajectories from \mbox{$t_\mathrm{s} - 1\,$s} until the cyclists leave the field of view (FOV) were used and for the waiting network, trajectories between \mbox{$t_\mathrm{w} + 1\,$s} and \mbox{$t_\mathrm{s} - 1\,$s} were used. The networks were trained using the Resilient Backpropagation (RPROP) \cite{Riedmiller.1993} algorithm.

Tab. \ref{tab:polynomials} shows the chosen parameters for the in- and output polynomials of the MLPs. The MLP consists of two hidden layers with 20 neurons in the first and 10 neurons in the second layer. A coarse-to-fine grid search was performed, to find the optimal network structure.

\begin{figure}
	\includegraphics[width=0.5\textwidth]{images/mlp_in_output_2.png}
	\caption{Example for in- and output of MLP: cyclist head velocity (gray), current time $t_\mathrm{c} = 2.0\,$s (green), input polynomials (black), output polynomials (ochre). }
	\label{fig:MLP_IN_OUT}
\end{figure}



==> sections/results_basic_movement_forecast.tex <==
\subsection{Movement Primitive Detection}

In this section we evaluate and compare different models optimized to detect movement primitives based on smart devices, infrastructure, and cooperation.

For training and evaluation of the classifier a $5$ fold cross-validation over the test subjects is performed. Hence, 
training and test subjects are disjunctive. In order to optimize the classifiers hyperparameters, $30\%$ of each training fold are retained and used as the validation set, while the other $70\%$ are used to train the model. Hyperparameters to be optimized are $C$ and $\gamma$ of the SVM as well as the class weight $cl_{w}$ used for training.

\begin{figure}[h]
	\includegraphics[clip, trim=0 0.3cm 0 0.3cm, width=0.5\textwidth]{images/start_wait_f1_score_delay.pdf}
	\vskip 3mm
	\caption{Weighted F1 score and delay of selected models. (Green: smartphone, Magenta: head trajectory 
		and Yellow: cooperative approach.)}
	\label{fig:f1score_delay}
	\vskip -6mm
\end{figure}

Fig.~\ref{fig:f1score_delay} shows the weighted F1 score of different models plotted over the delay axis with 
various parameter settings on the test set. 
The movement primitive classifiers for smart device (S), head trajectory (H), and cooperative movement primitive classifier (C) 
are selected ($10$ models each) from the Pareto front of the weighted F1 score and delay evaluated on the validation set. 
The reported classification statistics are obtained by evaluation of the selected models on the test set 
and without consideration of the probability calibration, i.e. direct class outcome of the SVM. 
The elements of the confusion matrix plus the delay of nine selected classifiers ($3$ of each) are denoted in the last five columns of Tab~\ref{tab:motion_primitive_results}. The statistics of the confusion matrix are weighted in the same fashion as the F1 score. 

{
	\setlength{\abovecaptionskip}{5pt plus 3pt minus 3pt}
	\begin{table}[b]
		\vskip -4mm
		\begin{center}
			\caption{Classification results of selected SVM with RBF kernel according to the multi-objective parameter optimization.} 
			\resizebox{8.4cm}{!}{
			\begin{tabular}{| c | c | c | c || c | c | c | c | c | c |}
				\hline
				ID & $C$ &  $\gamma$ & $cl_{w}$ & TP & TN & FP & FN & Delay $[\text{ms}]$\\ \hline \hline
				S1 & $2^9$ & $2^{-7}$ & $22$ & $0.994$ & $0.911$ & $0.093$ & $0.006$ & $32$ \\ \hline
				S2 & $2^{-1}$ & $2^{-4}$ & $15$ & $0.996$ & $0.918$ & $0.086$ & $0.003$ & $44$ \\ \hline
				S3 & $2^{-3}$ & $2^{-4}$ & $7$ & $0.992$ & $0.940$ & $0.063$ & $0.007$ & $106$ \\ \hline \hline
				H1 & $2^{-3}$ & $2^{-7}$ & $40$ & $0.996$ & $0.906$ & $0.099$ & $0.004$ & $54$ \\ \hline
				H2 & $2^{-5}$ & $2^{-3}$ & $7$ & $0.992$ & $0.969$ & $0.033$ & $0.008$ & $222$ \\ \hline
				H3 & $2^{-1}$ & $2^{-5}$ & $5$ & $0.989$ & $0.978$ & $0.023$ & $0.011$ & $246$ \\ \hline \hline
				\textbf{C1} & $\boldsymbol{2^{-7}}$ & $\boldsymbol{2^{-3}}$ & $\boldsymbol{7}$ & $0.995$ & $0.964$ & $0.039$ & $0.004$ & $96$ \\ \hline
				C2 & $2^{-3}$ & $2^{-1}$ & $27$ & $0.994$ & $0.958$ & $0.045$ & $0.006$ & $94$ \\ \hline
				C3 & $2^{1}$ & $2^{-7}$ & $10$ & $0.992$ & $0.978$ & $0.024$ & $0.007$ & $112$ \\ \hline
			\end{tabular}}
			\label{tab:motion_primitive_results}
		\end{center}	
%		\vskip -8mm
	\end{table}
}

We observe that classifiers based on the smart device activity data have small delays but 
a high false positive rate as compared to the classifiers based on head trajectories. 
For the latter the false positive rate is lower, going 
along with a higher delay. The three classifiers $S1$ to $S3$ and $H1$ to $H3$ are representatives which range from highly sensitive with 
a high false positive rate to rather slow starting detection behavior with a low false positive rate. 
A combination of these classifiers in pairs of two are used to create the cooperative classifier as described in Sec.~\ref{sec:cooperative_mp_pred}.
The hyperparameter of the cooperative classifier are again optimized using a grid search over the parameter space.
Selected classifiers are depicted in Fig.~\ref{fig:f1score_delay} and Tab.~\ref{tab:motion_primitive_results}.
The cooperative approach trades off a low false positive rate while retaining a fast starting detection time, i.e. low delay ($<100\,$ms).
The selected cooperative classifier $C1$ for further evaluation of the trajectory forecast 
is depicted in bold in Tab.~\ref{tab:motion_primitive_results}. It is a combination of a sensitive smart device classifier $S1$, which 
reacts upon the smallest movements (e.g. first instance of beginning pedaling movement), and a conservative head trajectory classifier $H3$. It detects the starting intention after $96\,$ms with an accuracy of $90\%$ and the accuracy reaches $95\,\%$ after $212\,$ms.


==> sections/results_prediction.tex <==
\subsection{Trajectory Forecast}

In this section, we compare the results of the combined approach including cooperative movement primitives detection and the trained MLPs for trajectory forecast. When tested only on starting motions, the starting forecast MLP model showed an $\mathit{ASAEE}$ of $0.379\, \frac{m}{s}$ compared to an $\mathit{ASAEE}$ of $0.507\,\frac{\text{m}}{\text{s}}$ of the model trained for all motion types without consideration of any movement primitives. In the following, the latter model is referred to as no movement primitive model (NP model). The model trained with only waiting scenes showed an $\mathit{ASAEE}$ of $0.042\,\frac{\text{m}}{\text{s}}$ compared to the NP model with $0.074\,\frac{\text{m}}{\text{s}}$ when tested on waiting scenes.

In Tab.~\ref{tab:asaee_results} the $\mathit{ASAEE}$ for different forecasting models and combinations of the soft gating approach with different movement primitive classifiers are reported.
The columns are the evaluation scenes (e.g. starting, waiting, or complete). 
The best performing forecasting model concerning the $\mathit{ASAEE}$ for all scenes is marked bold.
We observe that the values of $\mathit{ASAEE}$ over the complete scenes are close, 
and strongly dominated by waiting scenes, whereas for the starting scenes there is  
a strong difference between the performance of the models. 
Contrary to the results of the movement primitive detection (Tab.~\ref{tab:motion_primitive_results}), models which have a low delay perform worse than those which are slower but have a higher weighted F1 score (Fig. \ref{fig:f1score_delay}). 
This is because the probability for the starting class increases fast to a value above $0.5$ but 
then only slowly increases to $1.0$. Therefore, the forecast is dominated by a mixture of starting and 
waiting, making it effectively worse. 
%, than a model with lower delay but a sharper increase in the class model probability. 
The cooperative movement primitive detection can alleviate this problem, leading to a reduced $\mathit{ASAEE}$ for starting motions. 

{
	\setlength{\abovecaptionskip}{5pt plus 3pt minus 3pt}
	
	\begin{table}
		\begin{center}
			\caption{$\mathit{ASAEE}$ for different forecasting models} 
			\begin{tabular}{|p{1.7cm} | c | c | c |}
				\hline
				Model ID & Starting $[\text{m}/\text{s}]$ &  Waiting $[\text{m}/\text{s}]$ & Complete $[\text{m}/\text{s}]$ \\ \hline \hline
				S1 & $0.460$ & $0.047$  & $0.219$ \\ \hline
				S2 & $0.430$ & $0.053$ & $0.214$ \\ \hline
				S3 & $0.421$ & $0.052$ & $0.212$ \\ \hline \hline
				H1 & $0.432$ & $0.044$ & $0.211$  \\ \hline
				H2 & $0.412$ & $0.046$ & $0.207$ \\ \hline
				H3 & $0.424$ & $0.043$ & $0.209$ \\ \hline \hline
				\textbf{C1} & $\boldsymbol{0.403}$ & $\boldsymbol{0.043}$ & $\boldsymbol{0.201}$ \\ \hline
				C2 & $0.420$ & $0.041$ & $0.206$ \\ \hline
				C3 & $0.414$ & $0.044$ & $0.205$ \\ \hline \hline
				Starting Model & $0.379$ & - & - \\ \hline
				Waiting Model & - & $0.042$ & - \\ \hline
				NP Model & $0.507$ & $0.074$ &  $0.233$ \\ \hline
			\end{tabular}
			\label{tab:asaee_results}
		\end{center}	
		\vskip -6mm
	\end{table}
}

%\vskip 0.158cm
In Fig.~\ref{fig:AEE_starting}, the $\mathit{AEE}$ of all starting motions for forecast horizons from $0.02\,$s to $2.5\,$s after the labeled starting point are shown. In Fig.~\ref{fig:ASAEE_starting}, the $\mathit{ASAEE}$ of the forecast models over a time span of $2.5\,$s after the labeled starting point at $t=0$ is shown. 
% is shown by generating the AEE of the models at every time step $t$ and calculating the $\mathit{ASAEE}$ using Eq. \ref{eq:$\mathit{ASAEE}$}. 
For each time step $t$ a single $\mathit{ASAEE}$ value is calculated using Eq.~\ref{eq:ASAEE}. This is done by generating the $\mathit{AEE}$ for each forecast starting at time step $t$ with a forecast horizon of $2.5\,$s. 
Since it takes different amounts of time for the cyclists to leave the FOV of the cameras, not every trajectory could be used to evaluate the forecasts, especially at higher start times of the forecast. Table \ref{tab:samples_at_time} shows the number of samples used to generate the $\mathit{ASAEE}$ at different time steps.

\begin{table} [t]
%	\vskip -4mm
	\caption{Number of samples at a given time after start time}
	\begin{center}
		\vskip -0.5cm
		\resizebox{8.7cm}{!}{
			\begin{tabular}{ | l | c | c | c | c | c | c | }
				\hline
				Time & 0.0 s & 0.5 s & 1.0 s & 1.5 s & 2.0 s & 2.5 s \\ \hline
				Samples & 79 & 75 & 64 & 52 & 45 & 26 \\
				\hline
			\end{tabular}}
		\end{center}
		\label{tab:samples_at_time}
		\vskip -4mm
	\end{table}

\begin{figure}
	\begin{center}
		
		\subfigure[$\mathit{AEE}$ of starting scenes.]
		{
			\includegraphics[clip, trim=0 10 0 0]{images/start_aee.pdf}
			\label{fig:AEE_starting}
		} 
%		\vspace{-0.25cm}
		\subfigure[$\mathit{ASAEE}$ of starting scenes. Labeled starting point at $t=0$. ]
		{
			\includegraphics[clip, trim=0 10 0 10]{images/start_asaee_over_time.pdf}
			\label{fig:ASAEE_starting}
		}      % no label/numbering
%		\vspace{-0.25cm}
		\subfigure[$\mathit{AEE}$ of complete scenes.]
		{
			\includegraphics[clip, trim=0 10 0 0]{images/balanced_aee.pdf}
			\label{fig:AEE_complete}
			
		}
		
		\subfigure[$\mathit{AEE}$ waiting scenes.]
		{
			\includegraphics[clip, trim=0 10 0 0]{images/wait_aee.pdf}
			\label{fig:AEE_waiting}
		}
	\end{center}
	\vspace{0.2cm}
	\caption[] {$\mathit{ASAEE}$ and $\mathit{AEE}$ of predicted motions over a prediction horizon of $2.5\,$s (Dashed Blue: reference model given perfect movement primitive classification using starting or waiting model, respectively, Red: NP model, Green: model using smart device classifier (S2), Magenta: model using head trajectory classifier (H2), Yellow: model using cooperative movement primitive detection (C1)).}
\end{figure}

We observed that the NP model was outperformed by the starting model over the whole time span~(Fig.~\ref{fig:ASAEE_starting}). 
The starting model shows a much lower error during the first seconds after the starting point, for starting motions it is considered as the reference model.
We observe that all forecasting models in Fig.~\ref{fig:ASAEE_starting} 
using movement primitives to select between forecasting models perform better than the NP model. 
Moreover, the model using cooperative movement primitive detection shows the lowest initial $\mathit{ASAEE}$ and 
quickly converges towards the starting model. Especially in the first few hundred milliseconds, it slightly outperforms the model using head trajectory based movement primitive detection. 
This gain gets more stressed out when it is seen against the background of having manually labeled head tracks. 
If an automatic head detector and tracker is used, the head trajectory based classifier performance will decrease, 
attenuating the effects of cooperation.

Given perfect knowledge about movement primitives the maximal achievable $\mathit{ASAEE}$ with the approach 
of using movement primitives to select between models is $0.203\,\frac{\text{m}}{\text{s}}$.
This model is considered to be the reference model over the complete scenes.
Although having minor improvement opportunities at the detection of the starting point, 
the approach using cooperative movement primitives detection is able to beat the respective reference model over the 
complete scenes and can even improve on it with an $\mathit{ASAEE}$ of  $0.201\,\frac{\text{m}}{\text{s}}$. 
In Fig.~\ref{fig:AEE_complete}, this can be seen in the $\mathit{AEE}$ of the complete scenes. 
Here, the plots of the reference model and the cooperative approach are lying on top of each other.
The reason for this is that in some cases the cooperative approach detects the intention of the cyclist even 
before the labeled starting point and therefore decreases the forecasting error.
Moreover, the labeling of the starting point is not always unambiguous, e.g. the human operator interprets 
minor movements as waiting where there is still little movement. 
For such situations a mixture of the waiting and starting forecast models performs better 
than solely the forecast of the waiting model.
This can be seen best in Fig.~\ref{fig:AEE_waiting} showing the $\mathit{AEE}$ over the waiting scenes. 
For the waiting case the cooperative approach performs even better than the reference model for waiting scenes 
given perfect movement primitive classification.



%\begin{figure}[h]
%	
%	\caption{AEE of starting motions over a prediction horizon of 2.5 s (Blue: Start model, Red: NP model, Green: model using smart device classifier (S2), Magenta: model using head trajectory classifier (H2), Yellow: model using cooperative motion primitive detection (F1)).}
%
%\end{figure}

%\begin{figure}[h]
%	\includegraphics[width=0.5\textwidth]{images/balanced_aee.pdf}
%	\label{fig:AEE_complete}
%	\vskip -0.5cm
%	\includegraphics[width=0.5\textwidth]{images/wait_aee.pdf}
%	\caption{AEE of predicted complete and waiting scenes (Blue: Start model, Red: NP model, Green: model using smart device classifier (S2), Magenta: model using head trajectory classifier (H2), Yellow: model using cooperative motion primitive detection (F1)).  }
%	\label{fig:AEE_waiting}
%\end{figure}






==> sections/results_trajectories.tex <==
\subsection{Data Acquisition}
\label{sec_data_acquisition}
The developed algorithms are evaluated in experiments conducted with 49 female and male test subjects in the age between $18$~-~$54$.
The test subjects were equipped with a smart device and were instructed to move between certain points at an intersection while following the traffic rules. This resulted in 79 starting motions due to 2 traffic lights at the intersection. 
The smartphone is a Samsung Galaxy S6. It is carried in the trouser front pocket.
The intersection is  equipped with different sensors recording the test subjects. A complete description of the research intersection can be found in \cite{GoldhammerIntersection.2012}. To record the cyclist trajectories, a wide angle stereo camera system consisting of 2 high definition cameras ($1920 \times 1080\,$px, $50\,$fps) was used to track the head positions of the cyclist. The timestamps of the smartphone and the research intersection are synchronized offline.

\subsection{Trajectory Extraction}
\label{sec_results_trajectory_generation}
The head tracks on the video cameras are labeled by a human operators and are assumed to be close to the ground truth. The labeled positions are triangulated to obtain the 3D positions. In Fig.~\ref{fig:trajectories}, the extracted trajectories are plotted. The intersecting FOV of both cameras is shown in gray. The cyclists either started on the bicycle path on the road or on the sidewalk stopping at the traffic light and starting after the lights turn green to cross the street. The timespan of a scene is at most $14\,$s, i.e. $7\,$s before and after the starting point.

\begin{figure} [h]
	\includegraphics[width=0.5\textwidth]{images/trajectories.png}
	\vskip 3mm
	\caption{Overview of the intersection with all starting movements. The arrow is pointing into the starting direction. }
	\label{fig:trajectories}
	\vskip -0.3cm
\end{figure}

%The starting point is defined as the point in time at which the 
%rear wheel starts to move and a subsequent forward motion is recognizable. The starting points are labeled by human operators. 

